Data-Driven Fault Diagnosis Analysis and Open-Set Classification of Time-Series Data

Fault diagnosis of dynamic systems is done by detecting changes in time-series data, for example residuals, caused by system degradation and faulty components. The use of general-purpose multi-class classification methods for fault diagnosis is complicated by imbalanced training data and unknown fault classes. Another complicating factor is that different fault classes can result in similar residual outputs, especially for small faults, which causes classification ambiguities. In this work, a framework for data-driven analysis and open-set classification is developed for fault diagnosis applications using the Kullback-Leibler divergence. A data-driven fault classification algorithm is proposed which can handle imbalanced datasets, class overlapping, and unknown faults. In addition, an algorithm is proposed to estimate the size of the fault when training data contains information from known fault realizations. An advantage of the proposed framework is that it can also be used for quantitative analysis of fault diagnosis performance, for example, to analyze how easy it is to classify faults of different magnitudes. To evaluate the usefulness of the proposed methods, multiple datasets from different fault scenarios have been collected from an internal combustion engine test bench to illustrate the design process of a data-driven diagnosis system, including quantitative fault diagnosis analysis and evaluation of the developed open set fault classification algorithm.

==> method.tex <==
\section{Open Set Classification for Fault Diagnosis}
\label{sec:classification}

Since there could be multiple fault modes that could explain an observation 
$\bar{r}$ with pdf $p$, a conventional multi-class classifier is not suitable. 
To handle both that training data is not representative of all fault classes and 
that the objective is to identify not only the most likely diagnosis candidate but all 
diagnosis candidates, an open set fault classification algorithm is developed.   

A one-class classifier is designed for each fault class $f_i$ based on the modeling 
of fault modes and the approximated distinguishability measure \eqref{eq:dij}, such that 
a pdf $p$ can be explained by fault class $f_i$ if 
\begin{equation}
\mathcal{D}_{i}(p) = \min_{q \in \hat{\Omega}_i} K(p \| q) \leq J_i
\label{eq:fi_classifier}
\end{equation}
where $J_i$ is a threshold. The set $\hat{\Omega}_i$ is estimated from training 
data. Here, residual data is partitioned into fixed intervals and $p$ is estimated as 
a multivariate normal distributed fit to each interval. Note that more flexible 
distributions could be used at the cost of increased computational cost and 
numerical approximation of computing \eqref{eq:fi_classifier}. 

\subsection{Fault Mode Data Clustering}
Evaluating \eqref{eq:fi_classifier} requires a search over all elements in $\hat{\Omega}^c_i$.
Hierarchical clustering can be used to divide the search space such that 
\eqref{eq:fi_classifier} can be solved without having to evaluate all pdfs in $\hat{\Omega}^c_i$.
 
For example, the set $\hat{\Omega}_i$ can be clustered using a subset 
$\hat{\Omega}^c_i \subseteq \hat{\Omega}_i$ such that 
$\min_{q \in \hat{\Omega}^c_i} K(p \| q) \leq J_i$ for all 
$p \in \hat{\Omega}_i$. This subset can be approximated using, for example, 
the generalized $ k $-median clustering suggested in \cite{Ackerman2010clustering}.
Then, \eqref{eq:fi_classifier} can be evaluated by first evaluating all $\hat{\Omega}^c_i$
and then only continue evaluating the elements in the corresponding clusters 
that are close to $p$.

\subsection{Summary}
\label{sec:classification:summary}
For each new $p$:
\begin{itemize}
\item If $\mathcal{D}_{NF}(p) \leq J_i$ then $NF$ is the diagnosis output
\item else, for each fault mode $f_i$:
\begin{itemize}
\item $f_i$ is a diagnosis candidate if $\mathcal{D}_i(p) \leq J_i$
\end{itemize}
\item else if $\mathcal{D}_i(p) > J_i$ for all fault modes $f_i$, then the unknown fault case is the diagnosis candidate
\end{itemize}

The open set fault classifier can be improved incrementally as new data from different fault scenarios are collected and labelled, by updating the corresponding fault classes accordingly. 
